PTQ4SAM: Post-Training Quantization for Segment Anything

Segment Anything Model (SAM) has achieved impressive performance in many computer vision tasks. However, as a large-scale model, the immense memory and computation costs hinder its practical deployment. In this paper, we propose a post-training quantization (PTQ) framework for Segment Anything Model, namely PTQ4SAM. First, we investigate the inherent bottleneck of SAM quantization attributed to the bimodal distribution in post-Key-Linear activations. We analyze its characteristics from both per-tensor and per-channel perspectives, and propose a Bimodal Integration strategy, which utilizes a mathematically equivalent sign operation to transform the bimodal distribution into a relatively easy-quantized normal distribution offline. Second, SAM encompasses diverse attention mechanisms (i.e., self-attention and two-way cross-attention), resulting in substantial variations in the post-Softmax distributions. Therefore, we introduce an Adaptive Granularity Quantization for Softmax through searching the optimal power-of-two base, which is hardware-friendly. Extensive experimental results across various vision tasks (instance segmentation, semantic segmentation and object detection), datasets and model variants show the superiority of PTQ4SAM. For example, when quantizing SAM-L to 6-bit, we achieve lossless accuracy for instance segmentation, about 0.5\% drop with theoretical 3.9$\times$ acceleration. The code is available at \url{https://github.com/chengtao-lv/PTQ4SAM}.

==> sec/sub_sec/discriminator.tex <==
% 名称太朴素 KDE(Kernel Density Estimation)-based
\subsection{Histogram-based Discriminator} % 图片
\label{sec:discriminator}
However, not all activations after the key linears is bimodal distribution. To address this, we specifically design a histogram-based discriminator to distinguish it. Intuitively, we assume the process mainly consists two steps: to begin with, compared with Uniform distribution, Bimodal distribution is characterized by the existence of bell-shaped areas. Besides, compared with Normal distribution, the center of Bimodal distribution exhibits aforementioned void/sparse interval. Therefore, the aim of the discriminator is to detect bell-shaped area and void/sparse interval.

Frequency histograms can describe the distribution of activations. Divide the interval $[\min (\bf{x}), \max (\bf{x})]$ equally into $n$ bins as: 

\begin{equation}
    \left[\min (\bf{x}), \max (\bf{x})\right] =\left[x_0, x_1\right]\cup \left(x_1, x_2\right]\cup  \ldots\cup \left(x_{n-1}, x_n\right]
\end{equation}

The frequency of activation values in each bin is approximately equal to the probability of occurrence.

\begin{equation}
    P_i = P\left\{x_{i-1}<X \leq x_i\right\} 
\end{equation}
% Sort all the probabilities to get the top-k largest probabilities, ensuring that their sum is greater than a certain threshold.

We accumulate the top-k largest probability values to verify the bell-shaped area, written as
\begin{equation}
\label{eq:single}
    \sum_{top-k}P_i \ge \theta
\end{equation}
% Cluster the index values corresponding to the top-k largest probability values to obtain two sets. The clustering centers are recorded as $I_N$ and $I_P$, and the corresponding radii are $R_N$ and $R_P$. The distance between the two sets can represent the central void/sparse interval, that is

To find the left bound and right bound of the void/sparse interval, we cluster the index values of the top-k largest probability values to obtain two sets. Then we utilize the two sets to represent the distance, written as

\begin{equation}
\label{eq:dis}
    \|I_P-I_N\| - (R_P+R_N) \geq \eta * N
\end{equation}
where $I_N$ and $I_P$ denote the clustering centers of negative peak and positive peak, and $R_N$ and $R_P$ indicate the corresponding radii. If the distribution satisfies both Eq. \ref{eq:single} and Eq. \ref{eq:dis}, it is considered to be a Bimodal distribution.

% When its proportion is greater than a certain threshold $\eta$, the special Bimodal Distribution can be determined.

\begin{figure*}[]
    \centering
    \includegraphics[width=1\linewidth]{figure/framework.pdf}
    \caption{Illustration of our proposed PTQ4SAM. The Equivalent Sign Operation eliminates the bimodal distribution by simultaneously multiplying a channel-wise $\boldsymbol{\gamma}$ to both the query linear and key linear. The adaptive base logarithmic quantizer is employed for post-softmax activations.}
    \label{fig:frame}
\end{figure*}



==> sec/sub_sec/discriminator_ch.tex <==
% 名称太朴素
\subsection{Histogram-based Discriminator} % 图片
\label{sec:discriminator}
The special Bimodal Distribution in Figure \ref{fig:box} is only found in certain attention blocks. In order to eliminate the central void/sparse interval with the help of its special sign-consistent characteristics, we propose a Histogram-based discriminator to discriminate the Bimodal Distribution. Frequency histograms can describe the distribution of activations. Divide the interval $[\min (\bf{x}), \max (\bf{x})]$ equally into $N$ small bins as: 
% 两个公式，并集+p约等于fi

\begin{equation}
    \left[\min (\bf{x}), \max (\bf{x})\right] =\left[x_0, x_1\right]\cap\left(x_1, x_2\right]\cap \ldots\cap\left(x_{n-1}, x_n\right]
\end{equation}
The frequency of activation values in each interval is approximately equal to the probability of occurrence.
\begin{equation}
    P_i = P\left\{x_{i-1}<X \leq x_i\right\} 
\end{equation}
Sort all the probabilities to get the top-k largest probabilities, ensuring that their sum is greater than a certain threshold.
\begin{equation}
    \sum_{top-k}P_i \ge \theta
\end{equation}
Cluster the index values corresponding to the top-k largest probability values to obtain two sets. The clustering centers are recorded as $I_N$ and $I_P$, and the corresponding radii are $R_N$ and $R_P$. The distance between the two sets can represent the central void/sparse interval, that is
\begin{equation}
\label{eq:dis}
    \|I_P-I_N\| - (R_P+R_N) \geq \eta * N
\end{equation}
When its proportion is greater than a certain threshold $\eta$, the special Bimodal Distribution can be determined.

\begin{figure*}[]
    \centering
    \includegraphics[width=1\linewidth]{figure/framework.pdf}
    \caption{Illustration of our proposed PTQ4SAM. The Equivalent Sign Operation eliminates the bimodal distribution by simultaneously multiplying a channel-wise $\boldsymbol{\gamma}$ to both the query linear and key linear. The adaptive base logarithmic quantizer is employed for post-softmax activations.}
    \label{fig:frame}
\end{figure*}


